A two-step surrogate method for sequential uncertainty quantification in high-dimensional inverse problems

Predictive estimation, which comprises model calibration, model prediction, and validation, is a common objective when performing inverse uncertainty quantification (UQ) in diverse scientific applications. These techniques typically require thousands to millions of realisations of the forward model, leading to high computational costs. Surrogate models are often used to approximate these simulations. However, many surrogate models suffer from the fundamental limitation of being unable to estimate plausible high-dimensional outputs, inevitably compromising their use in the UQ framework. To address this challenge, this study introduces an efficient surrogate modelling workflow tailored for high-dimensional outputs. Specifically, a two-step approach is developed: (1) a dimensionality reduction technique is used for extracting data features and mapping the original output space into a reduced space; and (2) a multivariate surrogate model is constructed directly on the reduced space. The combined approach is shown to improve the accuracy of the surrogate model while retaining the computational efficiency required for UQ inversion. The proposed surrogate method, combined with Bayesian inference, is evaluated for a civil engineering application by performing inverse analyses on a laterally loaded pile problem. The results demonstrate the superiority of the proposed framework over traditional surrogate methods in dealing with high-dimensional outputs for sequential inversion analysis.

==> 05_Limitation.tex <==
\section{Additional remarks and limitations} \label{sec:limitation}
\begin{itemize}[left = 0cm]

 \item The proposed DR-based surrogate model is straightforward, only requiring a choice for the DR technique (e.g., PCA) and a surrogate (e.g., PCE). This feature is useful because the whole process is non-intrusive and does not require additional parameter tuning. 
 
 \item The implementation of the proposed surrogate modelling in this study exclusively focuses on PCA-PCE. It addresses dimensionality reduction (DR) solely through PCA and utilises Polynomial Chaos Expansion (PCE) for surrogate modelling. However, it's important to note that PCA-PCE is only one possible realisation to DR-surrogate modelling. Readers are encouraged to explore more advanced and nonlinear techniques beyond PCA-PCE.

 \item In this study, the DR-surrogate is only focusing on the high-dimensional outputs. Nonetheless, its potential effectiveness in managing high-dimensional inputs has been demonstrated and warrants exploration \cite{meles2022,kim2024,lataniotis2019,lataniotis2020}. Given the prohibitively high cost of finite element (FE) modelling and the challenge posed by the curse of dimensionality in input parameters, this study confines its focus to the output space. Future studies will contemplate the application of DR techniques in the high-dimensional input space.

 \item In an ideal scenario, it is speculated that DR-based surrogates maintain their superiority even in scenarios with lower dimensions. This is attributed to the belief that DR techniques extend beyond mere data compression; they can also leverage metrics that encompass covariance matrices and interconnections among outputs.

 \item Uncertainty arises from various sources, encompassing model discrepancy, observation error, parameter uncertainty, soil stochastic variability, etc. The whole framework is not limited to specific types of uncertainties. However, for simplicity and to better demonstrate the effectiveness of the proposed DR-based surrogate, observation errors and parameter uncertainties are assumed to be dominating the uncertainties. And observation errors are following a Gaussian distribution with constant variance $\sigma^2 \boldsymbol{I}$. Future endeavors by the authors will explore additional sources of uncertainty and consider relaxing the assumption of constant variance.

\end{itemize}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
